Facebook Political Ads And Accountability: Outside Groups Are Most Negative, Especially When Hiding Donors

The emergence of online political advertising has come with little regulation, allowing political advertisers on social media to avoid accountability. We analyze how transparency and accountability deficits caused by dark money and disappearing groups relate to the sentiment of political ads on Facebook. We obtained 430,044 ads with FEC-registered advertisers from Facebook's ad library that ran between August-November 2018. We compare ads run by candidates, parties, and outside groups, which we classify by (1) their donor transparency (dark money or disclosed) and (2) the group's permanence (only FEC-registered in 2018 or persistent across cycles). The most negative advertising came from dark money and disappearing outside groups, which were mostly corporations or 501(c) organizations. However, only dark money was associated with a significant decrease in ad sentiment. These results suggest that accountability for political speech matters for advertising tone, especially in the context of affective polarization on social media.

==> ethics.tex <==
\subsection{Ethics Checklist}

\begin{enumerate}

\item For most authors...
\begin{enumerate}
    \item  Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
    \answerYes{Yes}
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Yes}
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
    \answerYes{Yes, see the note about linear regression in the Analysis, as well the ``Limitations'' section of the Discussion}
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
    \answerYes{Yes, see the ``Federal Scope'' section of Data and Methods as well as the ``Limitations'' section of the Discussion}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, see the ``Limitations'' section of the Discussion}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Yes, see notes about affective polarization in the Introduction}
      \item Did you discuss any potential misuse of your work?
    \answerYes{Yes, see the ``Limitations'' section of the Discussion}
    \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
    \answerYes{Yes, see Data and Methods as well as the Appendix}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes}
\end{enumerate}

\item Additionally, if your study involves hypotheses testing...
\begin{enumerate}
  \item Did you clearly state the assumptions underlying all theoretical results?
    \answerYes{Yes, see Data and Methods}
  \item Have you provided justifications for all theoretical results?
    \answerYes{Yes, see Analysis}
  \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
    \answerYes{Yes, see hypotheses at the end of the Introduction}
  \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
    \answerYes{Yes, see the ``Limitations'' section of the Discussion}
  \item Did you address potential biases or limitations in your theoretical framework?
    \answerYes{Yes, see the ``Limitations'' section of the Discussion}
  \item Have you related your theoretical results to the existing literature in social science?
    \answerYes{Yes, see the Introduction}
  \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
    \answerYes{Yes, see the first part of the Discussion section}
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{NA}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{NA}
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
\item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? \answerNA{NA}
\item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)? \answerNA{NA}
\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)? \answerNA{NA}
\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? \answerNA{NA}
\item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made? \answerNA{NA}
\item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance? \answerNA{NA}
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
\item If your work uses existing assets, did you cite the creators?
\answerYes{Yes, see the ``Data Sources'' section of Data and Methods}
\item Did you mention the license of the assets?
\answerYes{Yes, see the ``Data Sources'' section of Data and Methods}
\item Did you include any new assets in the supplemental material or as a URL?
\answerYes{Yes, we will include our code (omitted for blind-review)}
\item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
\answerYes{Yes, see the ``Data Sources'' section of Data and Methods}
\item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
\answerNA{NA, no ad targeting or PII analyzed}
\item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR? \answerNA{NA}
\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset? \answerNA{NA}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
\item Did you include the full text of instructions given to participants and screenshots? \answerNA{NA}
\item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals? \answerNA{NA}
\item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation? \answerNA{NA}
\item Did you discuss how data is stored, shared, and deidentified? \answerNA{NA}
\end{enumerate}

\end{enumerate}

